Counterfactual Shapley Additive Explanations

Feature attributions are a common paradigm for model explanations due to their simplicity in assigning a single numeric score for each input feature to a model. In the actionable recourse setting, wherein the goal of the explanations is to improve outcomes for model consumers, it is often unclear how feature attributions should be correctly used. With this work, we aim to strengthen and clarify the link between actionable recourse and feature attributions. Concretely, we propose a variant of SHAP, Counterfactual SHAP (CF-SHAP), that incorporates counterfactual information to produce a background dataset for use within the marginal (a.k.a. interventional) Shapley value framework. We motivate the need within the actionable recourse setting for careful consideration of background datasets when using Shapley values for feature attributions with numerous synthetic examples. Moreover, we demonstrate the efficacy of CF-SHAP by proposing and justifying a quantitative score for feature attributions, counterfactual-ability, showing that as measured by this metric, CF-SHAP is superior to existing methods when evaluated on public datasets using tree ensembles.

==> tables/datasets_db_distance.tex <==
%auto-ignore
\begin{center}
    \begin{small}
        \begin{tabular}{llllll}
        \toprule
        Percentile of the Distance from the Decision Boundary &  100\% &  <50\% &  <20\% &  <10\% & <2.5\% \\
        Dataset                            &       &       &       &       &       \\
        \midrule
        GMSC (Give Me Some Credit)         &  4000 &  2000 &  2000 &  2000 &  1074 \\
        HELOC (Home Equity Line of Credit) &  4000 &  2000 &  1177 &   588 &   147 \\
        Lending Club (2007-2018)           &  4000 &  2000 &  2000 &  2000 &  2000 \\
        Wine Quality (White)               &  2996 &  1498 &   597 &   299 &    75 \\
        \bottomrule
        \end{tabular}
    \end{small}
\end{center}

